The Power of Priority Channel Systems

We introduce Priority Channel Systems, a new class of channel systems where messages carry a numeric priority and where higher-priority messages can supersede lower-priority messages preceding them in the fifo communication buffers. The decidability of safety and inevitability properties is shown via the introduction of a priority embedding, a well-quasi-ordering that has not previously been used in well-structured systems. We then show how Priority Channel Systems can compute Fast-Growing functions and prove that the aforementioned verification problems are $\mathbf{F}_{\varepsilon_{0}}$-complete.

==> app-upb.tex <==
\subsubsection*{A Finite Witness}
Observe that, if an execution
$C_0\hstep{}C_1\hstep{}C_2\hstep{}\cdots$ of the transition system
$\mathcal{S}_\#$ satisfies $C_i\leq_\# C_j$ for some indices $i<j$,
then because $\mathcal{S}_\#$ is a WSTS, we can simulate the steps
performed in this sequence after $C_i$ but starting from $C_j$ and
build an infinite run.  Conversely, if the system does not terminate,
\textit{i.e.}\ if there is an infinite execution
$C_0\hstep{}C_1\hstep{}C_2\hstep{}\cdots$, then because of the wqo we
will eventually find $i<j$ such that $C_i\leq_\# C_j$.  Therefore, the
system is non-terminating if and only if there is a finite witness of
the form
$C_0\hstep{*}C_i\hstep{+}C_j$ with $C_i\leq_\# C_j$.

\subsubsection*{Controlled Witnesses}
Another observation is that the size of successive configurations
cannot grow arbitrarily along runs; in fact, the length of the
channels contents can only grow by one symbol at a time using a write
transition.  This means that if we define
$|C=(q,x_1,\dots,x_m)|=\sum_{j=1}^m|x_j|$, then in an execution
$C_0\hstep{}C_1\hstep{}C_2\hstep{}\cdots$, $|C_i|\leq
|C_0|+i=H^i(|C_0|)$, \textit{i.e.}\ any execution is \emph{controlled} by the
successor function $H$.

\subsubsection*{Applying the Length Function Theorem}
\autoref{cor-lft} yields an \mbox{$h^{\Omega_{2(d+1)+1}}(|C_0|+|\Gamma|)$}
upper bound on the length of bad $(H,|C_0|)$-controlled sequences over
\mbox{$(\Sigma_{d,\Gamma}^\ast,\gpleq)$} for some polynomial $h$.  It can be
lifted to bound the maximal length of a witness in $\mathcal{S}_\#$,
when considering instead the ordinal
$o_{S}\eqdef(\Omega_{2(d+1)+1})^m\cdot|Q|$.  Setting
$|S|=|\Delta|+|Q|+d+m+|\Gamma|$, we see that this length is less than
$H^{\ez}\left(p(|S|+|C_0|)\right)<F_{\ez}\left(p(|S|+|C_0|)\right)$
for some fixed ordinal-recursive function $p$.

\subsubsection*{A Combinatorial Algorithm}
Since the functions $(h^\alpha)_{\alpha}$ are elementary
constructive~\citep[\theoremautorefname~5.1]{arXiv/Schmitz13}, the
above discussion yields a non-deterministic algorithm in $\F_{\ez}$
for Termination: compute $L=h^{o_{S}}(|C_0|+|\Gamma|)$ and
look for an execution of length $L+1$ in $\mathcal{S}_\#$.  If one
exists, it is necessarily a witness for nontermination; otherwise, the
system is guaranteed to terminate from $C_0$.

We call this a \emph{combinatorial} algorithm, as it relies on the
combinatorial analysis provided by the Length Function Theorem to
derive an upper bound on the size of a finite witness for the property
at hand---here Termination, but the same kind of techniques can be
used for Reachability and Inevitability.

